Detection of Clouds in Multiple Wind Velocity Fields using Ground-based Infrared Sky Images

Horizontal atmospheric wind shear causes wind velocity fields to have different directions and speeds. In images of clouds acquired using ground-based sky imagers, clouds may be moving in different wind layers. To increase the performance of an intra-hour global solar irradiance forecasting algorithm, it is important to detect multiple layers of clouds. The information provided by a solar forecasting algorithm is necessary to optimize and schedule the solar generation resources and storage devices in a smart grid. This investigation studies the performance of unsupervised learning techniques when detecting the number of cloud layers in infrared sky images. The images are acquired using an innovative infrared sky imager mounted on a solar tracker. Different mixture models are used to infer the distribution of the cloud features. The optimal decision criterion to find the number of clusters in the mixture models is analyzed and compared between different Bayesian metrics and a sequential hidden Markov model. The motion vectors are computed using a weighted implementation of the Lucas-Kanade algorithm. The correlations between the cloud velocity vectors and temperatures are analyzed to find the method that leads to the most accurate results. We have found that the sequential hidden Markov model outperformed the detection accuracy of the Bayesian metrics.

==> HMM.tex <==
\subsection{Hidden Markov Model}

A HMM is state space model which latent variables (i.e. system states) are discrete. In the problem of detecting the number of wind velocity fields in an image, a HMM is implemented to infer the cluster number $L$ in a mixture model. We assume that the current state of the system $L_t$ (i.e. cluster number) is a Markov process conditional to the previous observed states $p (L_t \mid L_{1}, \dots, L_{t - 1})$  \cite{BISHOP2006}. For simplification, we propose to model the process as a first-order Markov chain, which current state is only conditional to the immediately previous state $p (L_t \mid L_{1}, \dots, L_{t - 1}) = p (L_{t} \mid L_{t - 1}) $. Henceforth, $L$ is defined as the HMM hidden variable, which represents the number of detected wind velocity fields $L \in \{1, 2\}$ in image $L_t$, and $\mathbf{x}_{i,t}$ is an observations (i.e. feature vector).

The parameters $\boldsymbol{\theta}{}^{(l)}_t = \{ \pi{}^{(l)}_t, \boldsymbol{\mu}{}^{(l)}_t, \boldsymbol{\Sigma}{}^{(l)}_t \}$ of each distribution $l$ in the mixture model, and the hidden state of the system $L_t$ in image $t$ are the MAP estimation obtained applying the Bayes' theorem,
\begin{equation}
    \begin{split}
        \label{eq:bayes_theorem}
        p \left( \mathbf{z}_{i,t} \middle| \mathbf{x}_{i,t}, \boldsymbol{\Theta}_t \right) &= \frac{p \left( \mathbf{x}_{i,t}, \mathbf{z}_{i,t} \middle| \boldsymbol{\Theta}_t \right)}{p \left( \mathbf{x}_{i,t} \right)} \\
        &\propto p \left( \mathbf{x}_{i,t}, z^{(l)}_{i,t} \middle| \boldsymbol{\theta}_t^{(l)} \right) p \left( L_t \middle| L_{t - 1}  \right) \\
        &\propto p \left( \mathbf{x}_{i,t}, z^{(l)}_{i,t} \middle| \boldsymbol{\mu}_t^{(l)}, \boldsymbol{\Sigma}_t^{(l)} \right) p \left( \pi^{(l)}_t \middle| \boldsymbol{\alpha}^{(l)} \right) p \left( L_t \middle| L_{t - 1} \right).
    \end{split}
\end{equation}
The set with all the parameters in the mixture model in state $L_t$ are $\boldsymbol{\Theta}{}_t = \{ \pi{}^{(1)}_t, \boldsymbol{\mu}{}^{(1)}_t, \boldsymbol{\Sigma}{}^{(1)}_t, \dots, \pi{}^{(L_t)}_t, \boldsymbol{\mu}{}^{(L_t)}_t, \boldsymbol{\Sigma}{}^{(L_t)}_t  \}$, and the parameters of the prior distribution of the clusters weights $\pi^{(l)}$ are $\boldsymbol{\alpha}{}^{(l)}$.

The joint distribution $p ( \mathbf{x}_{i,t}, \mathbf{z}{}^{(l)}_{i,t} \mid \boldsymbol{\theta}{}^{(l)}_t ) = p ( \mathbf{x}_{i,t} \mid \mathbf{z}{}^{(l)}_{i,t}, \boldsymbol{\theta}^{(l)}_t ) p ( \mathbf{z}{}^{(l)}_{i,t} )$ is factorized to independently infer a mixture model of each feature,
\begin{equation}
    \begin{split}
        \label{eq:factorization}
        p \left( x_{i,t}^{(1)}, x_{i,t}^{(2)} \middle| z^{(l)}_{i,t}, \boldsymbol{\theta}_t^{(l)} \right) = p \left( x^{(1)}_{i,t} \middle| z^{(1,l)}_{i,t}, \boldsymbol{\theta}^{(l)}_{1,t} \right) p \left( x^{(2)}_{i,t} \middle|  x^{(1)}_{i,t}, z^{(1,l)}_{i,t}, z^{(2,l)}_{i,t}, \boldsymbol{\theta}^{(l)}_{2,t}\right) 
    \end{split}
\end{equation}
where $\boldsymbol{\theta}{}^{(l)}_t = \{ \mathbf{z}{}^{(l)}_{1,t}, \mathbf{z}{}^{(l)}_{1,t} \}$ and $\boldsymbol{\gamma}{}^{(l)}_t = \{ {z}{}^{(l)}_{1,t}, {z}{}^{(l)}_{2,t} \}$ are the parameters of the independent mixture models and the responsibilities respectively.

The posterior distribution of a mixture model is proportional to the joint probability of the observations $\mathbf{x}_{i,t}$ and the responsibilities $z{}^{(l)}_{i,t}$ of each cluster detected in image $t$. The state of the system $L_t$, which represents the number of clusters $L$ in the mixture models, is modelled using a HMM. Therefore, the mixture model parameters inferred using Eq. \eqref{eq:CDLL} is
\begin{equation}
    \label{eq:joint_distribution}
    p \left( \mathbf{X}_{t}, \mathbf{Z}^{(l)}_{t} \middle| \hat{\boldsymbol{\theta}}^{(l)}_t, \hat{\boldsymbol{\alpha}}^{(l)} \right) \triangleq \left\{ \sum^N_{i = 1} \left[ \prod^{L_t}_{l = 1} \left[  \pi^{(l)} p \left( \mathbf{x}_{i,t} \middle| \hat{\boldsymbol{\mu}}^{(l)}_t, \hat{\boldsymbol{\Sigma}}^{(l)}_t \right) \right]^{\mathbb{I} (z_{i,t} = l)} \right] \right\} p \left(\pi^{(l)} \middle| \hat{\boldsymbol{\alpha}}^{(l)}\right),
\end{equation}
where $\hat{\boldsymbol{\theta}}{}^{(l)}_t$ and $\hat{\boldsymbol{\alpha}}{}^{(l)}$ are the parameters that maximize the CDLL of the mixture model with $L_t$ clusters. 

The prior on the latent variable $L_t$, is defined as a distribution of the exponential family, 
\begin{equation}
    \label{eq:prior}
    \log p \left( L_t \middle| L_{t - 1} \right) = \frac{1}{Z} \exp \left[ - \psi \left( L_t, L_{t - 1}\right) \right],
\end{equation}
where the exponent $\psi ( L_t, L_{t - 1})$, is a function that depends on the previous state of the system $L_{t - 1}$,
\begin{equation}
    \psi \left( L_t, L_{t - 1} \right) \triangleq 
    \left\{
    \begin{array}{lll}
        -\beta & \text{if} & L_t = L_{t-1} \\ 
        +\beta & \text{if} & L_t \neq L_{t-1}
    \end{array} \right.
    \label{eq:hmm_prior},
\end{equation}
the parameter $\beta$ has to be cross-validated.

Combining Eq. \eqref{eq:joint_distribution} and Eq. \eqref{eq:prior} in Eq. \eqref{eq:bayes_theorem}, and taking logarithms and expectations with respect to $z_{i,t}$, the CDLL of a image $t$ being in state $L^{(t)}$ are,
\begin{equation} 
    \begin{split}
        %p \left( y_t \middle| \mathbf{X}_{t}, \hat{\boldsymbol{\theta}}_t^{(l)}, \hat{\boldsymbol{\alpha}}^{(l)} \right) &= \left\{\sum^L_{l = 1} \sum^N_{i = 1}\log \left[ \pi^{(l)} p \left( \mathbf{x}_{i,t} \middle| \hat{\boldsymbol{\mu}}^{(l)}_t, \hat{\boldsymbol{\Sigma}}^{(l)}_t \right) \right]^{\mathbb{I} \left( z_{i,t} = l \right)} \right\} \\
        %\log p \left( \boldsymbol{\gamma}_t \middle| \mathbf{X}_{t}, \hat{\boldsymbol{\theta}}_t^{(l)}, \hat{\boldsymbol{\alpha}}^{(l)}, L_t \right)
        \mathcal{Q} \left( \boldsymbol{\theta}, \boldsymbol{\theta}_{t - 1} \right) &= \left[ \sum^N_{i = 1} \sum^{L_t}_{l = 1} \gamma^{(l)}_{i,t} \log \pi^{(l)}_{t} + \sum^N_{i = 1} \sum^{L_t}_{l = 1} \gamma^{(l)}_{i,t} \log p \left( \mathbf{x}_{i,t} \middle| \boldsymbol{\theta}^{(l)}_t\right) \right] \\
        &\quad \quad \quad + \log p \left(\pi^{(l)} \middle| \hat{\boldsymbol{\alpha}}^{(l)}\right) - \psi \left( L_t, L_{t - 1} \right) + \mathrm{constant}.
    \end{split}
\end{equation}
It should be noted that $\psi \left( L_t, L_{t - 1} \right)$ is a constant with respect to $z_{i, t}$, so maximizing this equation is equivalent to maximizing the original CDLL in Eq. \eqref{eq:joint_distribution}.

After completing the inference of the mixture model parameters $\hat{\boldsymbol{\theta}}{}^{(l)}_t$ and $\hat{\boldsymbol{\alpha}}{}^{(l)}$ when $L_t = 1$ and $L_t = 2$, the optimal state of the system $\hat{L}_t \in \{ 1, 2\}$ is the MAP estimation obtained from,
\begin{equation}
    \hat{L}_t = \underset{L_t \in \{1, 2 \}}{\operatorname{argmax}} \ \left[ \sum_{i = 1}^N \sum_{l = 1}^{L_t} \log p \left( \mathbf{z}_{i,t} \middle| \mathbf{x}_{i,t}, \hat{\boldsymbol{\theta}}{}^{(l)}_t, \hat{\boldsymbol{\alpha}}{}^{(l)}, L_t \right) \right] - \psi \left( L_t, L_{t - 1} \right),
\end{equation}
where the latent variable $L_t$ defines the number of different wind velocity fields detected in an image.

==> PWLK.tex <==
\subsubsection{Lucas-Kanade Method}

The dimension of the image and the weights are reduced in proportion to scale-level of the number of pyramids applied in the implementation. The computed velocity vector in the pyramidal scale-levels are extrapolated to the the original dimensions of the image and average together. 

The LK method proposes to find the solution for the optical flow equations via Least Squares (LS). In this research, the LK method is extended to multiple pyramidal levels. In the first step, for each finite difference in Eq. \eqref{eq:finite_differences} a set of matrices  $\mathbf{I}^\prime = \{(\mathbf{I}_{x, 1}^\prime, \mathbf{I}_{y, 1}^\prime, \mathbf{I}_{t, 1}^\prime), \dots, (\mathbf{I}_{x, K}^\prime, \mathbf{I}_{y, K}^\prime, \mathbf{I}_{t, K}^\prime) \}$ is constructed, with resolution reduced in a factor $k\delta$, $1 \leq k \leq K$  where $1/\delta$ is the pyramid scale. A sliding window is defined with odd width $W = 2w+1$ and where $w$ is the window size parameter, to be cross-validated.

Now we assume that the image may contain more than one velocity field. Then, at pixel $i,j$ of layer $l$, we define $1 \leq l \leq L$ hypothesis over the possible velocities $\mathbf{v}^{(l)}_{i,j,k}$. 

If the position of the central pixel of the window is defined as $i,j$, then the dependent and independent variables can be defined as 
\begin{equation}
    \begin{split}
        \mathbf{x}_{i - m, j - n, k} &=
            \begin{bmatrix}
                \mathbf{I}^\prime_{x, k} \left(i - m, j - n \right) \\ 
                \mathbf{I}^\prime_{y, k} \left(i - m, j - n \right)
            \end{bmatrix}, \quad
        \mathbf{v}^{(l)}_{i, j,k} =
            \begin{bmatrix}
                u^{(l)}_{i, k} \\ 
                v^{(l)}_{j, k}
            \end{bmatrix}, \ 
        \\
        y_{i - m, j - n, k} &= -\mathbf{I}^\prime_{t, k} \left( i - m, j - n \right), \quad
        - w \leq m \leq  w, \quad - w \leq n \leq  w.
    \end{split}
\end{equation}
{\color{red} Posteriors have been defined two times in this section in different manners}
Each velocity is associated to a posterior probability $\gamma_{i,j,k}^{(l)} \triangleq  p ( z_{i,j,k} = l \mid T_{i,j})$ where $z_{i,j,k} = l$ is a latent variable that indicates that the velocity field at pixel $i,j$ of pyramid level $k$ is the one corresponding to cloud layer $l$. These posteriors will be estimated in the next section.
  
  

% In order to estimate the velocity vector ${\bf v}^{(l)}_{i,j,k}$, the mean square error $\mathbb{E}\left[e^2_{i,j,k}\right]$ of the linear equations set  
% \begin{equation}
%     {\bf v}^{(l)\top}_{i,j,k}{\bf x}_{i,j,k} = y_{i,j,k} - e_{i,j,k},
% \end{equation}
% is minimized for each pyramid level.

% % \begin{equation}
%     \mathbf{X}_{i,j,k} =
%         \begin{bmatrix}
%             \mathcal{I}_x \left( \mathbf{x}_1 \right) & \mathcal{I}_y \left( \mathbf{x}_1 \right) \\
%             \mathcal{I}_x \left( \mathbf{x}_2 \right) & \mathcal{I}_y \left( \mathbf{x}_2 \right) \\ 
%             \vdots                                    & \vdots \\ 
%             \mathcal{I}_x \left( \mathbf{x}_W \right) & \mathcal{I}_y \left( \mathbf{x}_W \right)
%         \end{bmatrix}; \ \ \ 
%     \mathbf{w}_{i,j,k} =
%         \begin{bmatrix}
%             v_x \\ 
%             v_y
%         \end{bmatrix}; \ \ \ 
%     \mathbf{y}_{i,j,k} =
%         \begin{bmatrix}
%             -\mathcal{I}_t\left( \mathbf{x}_1 \right) \\ 
%             -\mathcal{I}_t\left( \mathbf{x}_2 \right) \\ 
%             \vdots \\ 
%             -\mathcal{I}_t\left( \mathbf{x}_W \right)
%         \end{bmatrix}   
% \end{equation}

%Instead of the standard weighting of the neighboring pixels in the window using the probabilities of a normal distribution used in the pyramidal LK method, 
We introduce a Weighted Least Squares (WLS) approach \cite{SIMON2003}, whose weights are posterior probabilities $\gamma^{(l)}_{i,j,k}$. Assume an extended vector ${\bf y}_{i,j,k}$ containing all instances of  ${\bf y}_{i-m,j-n,k}$ and a matrix ${\bf X}_{i,j,k}$ containing all ${\bf x}_{i-m,j-n,k}$.

Instead of minimizing the mean square error, we can maximize the expectation of the unnormalized log-posterior 
\begin{equation}\label{eq:log_posterior}
    \begin{split}
    &\mathbb{E} \left\{\log \left[ p({\bf y}_{i,j,k} | {\bf X}_{i, j, k},{\bf v}^{(l)}_{i,j,k}) p({\bf v}^{(l)}_{i,j,k})\right] \right\} = \\
    &= \mathbb{E} \left\{ \log  \left[ \prod_{m,n,l} \left[ p({\bf y}_{i - m, j - n,k} | {\bf x}_{i - m,j - n,k}, {\bf v}_{i,j,k}^{(l)}) \right]^{\mathbb{I}(z_{i,j,k}= l) } p({\bf v}^{(l)}_{i,j,k}) \right] \right\} \\
    &= \sum_{m, n, l} \mathbb{E} \left[ \mathbb{I}( z_{i-m, j-n, k} = l)\right] \log p({\bf y}_{i - m, j - n,k} | {\bf x}_{i - m, j  -n, k}, {\bf v}_{i, j, k}^{(l)} )  + \log p({\bf v}^{(l)}_{i,j,k}) \\
    & = \sum_{m, n, l} \gamma^{(l)}_{i - m, j - n, k} \log p({\bf y}_{i - m, j - n, l}|{\bf x}_{i - m, j - n, k},{\bf v}^{(l)}_{i, j, k}) + \log p({\bf v}_{i, j, k}^{(l)}) \\
    &= - \sum_{m, n, l} \gamma^{(l)}_{i - m, j - n, k} \| {\bf v}^{(l)\top}_{i, j, k} {\bf x}_{i - m, j - n,k} - {\bf y}_{i - m, j - n, k}\|^2 - \tau \| {\bf v}^{(l)}_{i, j, k} \|^2 + \text{constant}
    \end{split}
\end{equation}
{\color{red} Here is the other}
where $\gamma^{(l)}_{i - m, j - n,k} = \mathbb{E}[ \mathbb{I}(z_{i - m, j - n, k} = l)]$ is the posterior probability of the velocity field, $\mathbb{I}(\cdot)$ is the indicator function, and where we assumed that both probabilities are Gaussian distributions, where the first one is a multivariate Gaussian modelling the error, which has a given variance $\sigma_n^2$, and the second one is a multivariate Gaussian modelling the prior over the velocities, whose covariance is an identity $\mathbf{I}_{2 \times 2}$. Thus, $\tau=\sigma_n^{2}$ plays the role of a regularization parameter, and it may be validated or inferred by maximizing the likelihood term \cite{sundararajan2000}.

By computing the gradient of the expression with respect to ${\bf v}^{(l)}_{i,j,k}$ and nulling it, we obtain the solution,
\begin{equation}
    \mathbf{v}^{(l)}_{i,j,k} = \left( \mathbf{X}_{i,j,k} \boldsymbol{\Gamma}_{i,j,k}^{(l)} \mathbf{X}_{i,j,k}^\top + \tau \mathbf{I}_{2L \times 2L} \right)^{-1} \mathbf{X}_{i,j,k} \boldsymbol{\Gamma}_{i,j,k}^{(l)} \mathbf{y}_{i,j,k}
\end{equation}
where ${\boldsymbol \Gamma}_{i,j,k}^{(l)}$ is a diagonal matrix containing all posteriors of the $l$ cluster. 

\iffalse
The analytical solution of the WLK problem for each coordinate $i,j$ in each pyramid level $k$ is
\begin{equation}
    \begin{split}
        \mathbf{X}_{i,j,k} \boldsymbol{\Gamma}_{i,j,k} \mathbf{X}_{i,j,k}^\top \mathbf{v}_{i,j,k} &= \mathbf{X}_{i,j,k} \boldsymbol{\Gamma}_{i,j,k} \mathbf{y}_{i,j,k} \\ 
        \mathbf{v}_{i,j,k} &= \left( \mathbf{X}_{i,j,k} \boldsymbol{\Gamma}_{i,j,k} \mathbf{X}_{i,j,k}^\top + \tau \mathbf{I}_{2 \times 2} \right)^{-1} \mathbf{X}_{i,j,k} \boldsymbol{\Gamma}_{i,j,k} \mathbf{y}_{i,j,k},
    \end{split}
\end{equation}
where ${\bf X}_{i,j,k}$ is a matrix containing all vectors ${\bf x}_{m,n,k}$ and ${\bf y}_{i,j,k}$ is a column vector containing all values $y_{n,m,k}$. To add $\tau$ to the diagonal of $\mathbf{X}_{i,j,k} \boldsymbol{\Gamma}_{i,j,k} \mathbf{X}_{i,j,k}^\top$ is equivalent to assure that the eigenvalues of the velocities are such as $\lambda_1 \geq \lambda_2 > \tau $, which is equivalent to regularize the velocities estimation.
\fi


% This might be an ill-conditioned problem. The eigenvalues of the covariance matrix are,
% \begin{equation}
%     \mathbf{X}_{i,j,k}^\top \boldsymbol{\Gamma}_{i,j,k} \mathbf{X}_{i,j,k} = \mathbf{1} \left[
%     \begin{array}{cc}{\lambda_1} & {0} \\ {0} & {\lambda_2}
%     \end{array} \right] \mathbf{1},
% \end{equation}
% where $\mathbf{1}$ is an unitary matrix of size $2 \times 2$, $\lambda_1$ and $\lambda_2$ has to be non-zero. 


The estimated velocity components are defined for each Euclidean coordinate in a pyramid level $k$ as $\mathbf{U}^{(l)}_k = \{ u^{(l)}_{i,j,k} \in \mathbb{R} \mid i = 1, \dots, N / k, \ j = 1, \dots,  M / k \} \in \mathbb{R}^{N / k \times M / k}$ and $\mathbf{V}^{(l)}_k = \{ v^{(l)}_{i,j,k} \in \mathbb{R} \mid i = 1, \dots, N / k, \ j = 1, \dots,  M / k \} \in \mathbb{R}^{N / k \times M / k}$. The velocity field is extrapolated to the original Euclidean frame of reference. The bilinear interpolation method is implemented to estimate the velocity component continuous functions \cite{SMITH1981}. The functions are defined as $\mathcal{U}: \mathbf{x} \mapsto u \in \mathbb{R}$, and $\mathcal{V}: \mathbf{x} \mapsto v \in \mathbb{R}$. After the application of the interpolation, the estimated velocity components are $\mathbf{U}^{(l)}_k \in \mathbb{R}^{N \times M}$ and $\mathbf{V}^{(l)}_k \in \mathbb{R}^{N \times M}$ for each pyramidal level. 

The velocity field in an image is computed averaging the velocity fields that were estimated in each one of the pyramids for each posterior $l$,
\begin{equation}
    \mathbf{U}^{(l)} = \frac{\sum^K_{k = 1} k \delta\mathbf{U}^{(l)}_{k}}{K}; \quad
    \mathbf{V}^{(l)} = \frac{\sum^K_{k = 1} k \delta \mathbf{V}^{(l)}_{k}}{K}.
\end{equation}
The obtained velocity components for each posterior $l$, are averaged weighting the vectors components by their posterior,
\begin{equation}
    \mathbf{U} = \sum_{l = 1}^L \left( \boldsymbol{\Gamma}^{(l)} \odot \mathbf{U}^{(l)} \right); \quad \mathbf{V} = \sum_{l = 1}^L \left( \boldsymbol{\Gamma}^{(l)} \odot \mathbf{V}^{(l)} \right),
\end{equation}
where $\odot$ is the Hadamard product. The result are the velocity components for each pair of coordinates in the original frame $\mathbf{U}, \mathbf{V} \in \mathbb{R}^{N \times M}$. The velocity vectors defined in polar coordinates have magnitude $\mathbf{R} = ( \mathbf{U} \odot \mathbf{U} + \mathbf{V} \odot \mathbf{V})^{1/2}$ and angle $\boldsymbol{\Phi} = \mathbf{arctan2} ( \mathbf{U}, \mathbf{V} )$.

%The mixture model used to infer the posterior  distribution $\mathbf{\Gamma}_{i,j,k}$ of the velocity vectors is expected to have multiple clusters when there are multiple wind velocity fields in the image. 

==> PWLK_1.tex <==
\begin{table}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{3.75pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.25} % Default value: 1
    \begin{tabular}{lcccccccccccccc}
        \toprule
        \multicolumn{10}{c}{PWLK Multiple Cloud Layers Detection Accuracy [\%]} \\
        \midrule
        \multicolumn{1}{c}{Univariate} & \multicolumn{5}{c}{Bayesian Metrics} & \multicolumn{3}{c}{Cross-Validated} & MAP-MRF \\
        \multicolumn{1}{c}{Likelihoods} & $\mathcal{Q}$ &  $\mathcal{BIC}$ & $\mathcal{AIC}$ & $\mathcal{CLC}$ & $\mathcal{ICL}$ & $\alpha_0$ & $\alpha_1$ & $\beta$ & $\psi \left( y^{(t)} = y^{(t - 1)} \right)$ \\
        \midrule
        $\mathcal{VM} ( \phi_{i,j} ) $ & 57.41 & 58.14 & 59.26 & 61.48 & 61.85 & - & 1 & 100 & 58.52 \\
        $\mathcal{G} ( r_{i,j} ) $ & 45.19 & 46.3 & 46.3 & 42.59 & 42.59 & - & 1 & 600 & 39.26 \\
        \bottomrule
    \end{tabular}
    \caption{Detection accuracy achieved when univariate probability functions are used in a mixture model likelihood and two pyramidal levels in the PWLK. The detection accuracy is compared using different Beyesian metrics and a mixture model with a prior on the weights and the clusters number.}
    \label{tab:univariate_mms}
\end{table}

==> PWLK_2.tex <==
\begin{table}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.35pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.25} % Default value: 1
    \begin{tabular}{lcccccccccccccc}
        \toprule
        \multicolumn{10}{c}{PWLK Multiple Cloud Layers Detection Accuracy [\%]} \\
        \midrule
        \multicolumn{1}{c}{Multivariate} & \multicolumn{5}{c}{Bayesian Metrics} & \multicolumn{3}{c}{Cross-Validated} & MAP-MRF \\
        \multicolumn{1}{c}{Likelihoods} & $\mathcal{Q}$ &  $\mathcal{BIC}$ & $\mathcal{AIC}$ & $\mathcal{CLC}$ & $\mathcal{ICL}$ & $\alpha_0$ & $\alpha_1$ & $\beta$ & $\psi \left( y^{(t)} = y^{(t - 1)} \right)$ \\
        \midrule
        $\mathcal{N} ( \mathbf{v}_{i,j} ) $ & 62.69 & 61.85 & 58.52 & 62.96 & 65.19 & - & 10 & 350 & 71.48 \\
        $\mathcal{N} ( T_{i,j}, \mathbf{v}_{i,j} )$ & 52.22 & 52.96 & 52.22 & 51.85 & 64.44 & 100 & - & 1000 & 74.07 \\
        $\mathcal{BG} ( \tilde{T}_{i,j}, r_{i,j} )$ & 50 & 50.37 & 50.37 & 50 & 50.37  & 1 & - & 0 & 50.37 \\
        $\mathcal{BG} ( \tilde{T}_{i,j}, r_{i,j} ) \mathcal{VM} ( \phi_{i,j} )$ & 50 & 50.37 & 50 & 50 & 49.63 & 1 & 1 & 0 & 50 \\
        $\mathcal{B} ( \bar{T}_{i,j} ) \mathcal{N} ( \mathbf{v}_{i,j} ) $ & $\mathbf{74.07}$ & $\mathbf{73.33}$ & $\mathbf{74.07}$ & $\mathbf{78.89}$ & $\mathbf{80.37}$ & 10 & 10 & 700 & $\mathbf{84.44}$ \\
        $\mathcal{G} ( \tilde{T}_{i,j} ) \mathcal{N} ( \mathbf{v}_{i,j} )$ & 64.07 & 65.19 & 64.07 &  59.26 & 53.70 & 10 & 100 & 600 & 69.29 \\
        \bottomrule
    \end{tabular}
    \caption{Detection accuracy achieved when multivariate probability functions are used in the likelihood of the mixture model and two pyramidal levels in the PWLK. The detection accuracy is compared using different Bayesian metrics and a maximum a posterior implementation of a mixture model with a prior on the weights and cluster numbers.}
    \label{tab:multivariate_mms}
\end{table}

==> PWLK_3.tex <==
\begin{table}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.35pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.25} % Default value: 1
    \begin{tabular}{lcccccccccccccc}
        \toprule
        \multicolumn{10}{c}{PWLK Multiple Cloud Layers Detection Accuracy [\%]} \\
        \midrule
        \multicolumn{1}{c}{Factorized} & \multicolumn{5}{c}{Bayesian Metrics} & \multicolumn{3}{c}{Cross-Validated} & MAP-MRF \\ \multicolumn{1}{c}{Univariate Likelihoods} & $\mathcal{Q}$ &  $\mathcal{BIC}$ & $\mathcal{AIC}$ & $\mathcal{CLC}$ & $\mathcal{ICL}$ & $\alpha_0$ & $\alpha_1$ & $\beta$ & $\psi \left( y^{(t)} = y^{(t - 1)} \right)$ \\
        \midrule
        $\mathcal{B} ( \bar{T}_{i,j} ) \mathcal{VM} ( \phi_{i,j} ) $ & 72.22 & 72.22 & 70 & $\mathbf{74.44}$ & $\mathbf{78.52}$ & 1 & 10 & 650 &$\mathbf{97.78}$ \\
        $\mathcal{B} ( \bar{T}_{i,j} ) \mathcal{G} ( r_{i,j} ) $ & 54.07 & 52.22 & 51.85 & 48.15 & 48.52 & 1 & 1000 & 1000 & 68.52 \\
        $\mathcal{B} ( \bar{T}_{i,j} ) \mathcal{VM} ( \phi_{i,j} ) \mathcal{G} ( r_{i,j} ) $ & 52.92 & 54.44 & 53.33 & 55.56 & 48.89 & 100 & 1000 & 1000 & 74.81 \\
        $\mathcal{G} ( \tilde{T}_{i,j} ) \mathcal{VM} ( \phi_{i,j} ) $ & 64.81 & 61.48 & 63.33 & 49.63 & 53.33 & 10 & 1000 & 500 & 68.89 \\
        $\mathcal{G} ( \tilde{T}_{i,j} ) \mathcal{G} ( r_{i,j} ) $ & 52.59 & 51.11 & 51.85 & 50 & 53.33 & 10 & 1 & 1000 & 64.81\\
        $\mathcal{G} ( \tilde{T}_{i,j} ) \mathcal{VM} ( \phi_{i,j} ) \mathcal{G}  ( r_{i,j} ) $ & 51.11 & 58.89 & 54.81 & 51.11 & 56.67 & 10 & 1 & 450 & 55.56 \\
        $\mathcal{N} ( T_{i,j} ) \mathcal{VM} ( \phi_{i,j} ) $ & $\mathbf{78.15}$ & $\mathbf{76.67}$ & $\mathbf{77.41}$ & 72.96  & 71.85 & 1000 & 1000 & 600 & 81.85 \\  
        $\mathcal{N} ( T_{i,j} ) \mathcal{G} ( r_{i,j} ) $ & 64.07 & 66.67 & 64.44 & 61.85 & 70.37 & 100 & 10 & 150 & 69.25 \\
        $\mathcal{N} ( T_{i,j} ) \mathcal{VM} ( \phi_{i,j} ) \mathcal{G} ( r_{i,j} ) $ & 73.33 &  67.78 & 68.15 &  72.96 & 68.89 & 1000 & 100 & 250 & 72.22 \\
        $\mathcal{VM} ( \phi_{i,j}) \mathcal{G} ( r_{i,j} ) $ & 47.04 & 48.15 & 47.04 & 48.52 & 45.56 & - & 1000 & 1000 & 60.74 \\
        \bottomrule
    \end{tabular}
    \caption{Detection accuracy achieved when the when the mixture model likelihood is factorized in the produce of independent likelihoods functions for each feature and two pyramidal levels in the PWLK. The detection accuracy is compared using different Bayesian metrics and adding a prior of the weights and the cloud layers number to mixture model.}
    \label{tab:factorize_univariate_mm}
\end{table}

==> table.tex <==
\begin{table}
\centering
\tiny
\setlength{\tabcolsep}{2.pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.75} % Default value: 1
\begin{tabular}{lcccccccccccccc}
\toprule
\multicolumn{10}{c}{Multiple Cloud Layers Detection Accuracy [\%]} \\
\midrule
{} & \multicolumn{5}{c}{Bayesian Metrics} & \multicolumn{3}{c}{Cross-Validated} & MAP-MRF \\
Mixture Model Likelihoods & $\mathcal{L}$ &  $\mathcal{BIC}$ & $\mathcal{AIC}$ & $\mathcal{CLC}$ & $\mathcal{ICL}$ & $\alpha_0$ & $\alpha_1$ & $\beta$ & $\psi \left( y^{(t)} = y^{(t - 1)} \right)$ \\ & & & & & & & & \\
\midrule
$\mathcal{B} \left( \bar{T}_{i,j} \mid \alpha_k, \beta_j \right)$ & 66.67 & 70.74 & 70.74   & 76.3 &  76.67 & 1 & - & 200 & 75.93 \\
$\mathcal{G} \left(  \tilde{T}_{i,j} \mid \alpha_k, \beta_k \right) $ & 60 & 61.11 & 60.74 & 66.67 & 70.74 & 1 & - & 300 & 53.55 \\
$\mathcal{N} \left(  T_{i,j} \mid \mu_k, \sigma_k \right) $ & 74.07 & 73.7 & 71.85 & $\mathbf{79.63}$ & $\mathbf{81.11}$ & 100 & - &  500 & 87.41 \\
$\mathcal{VM} \left(  \phi_{i,j} \mid \mu_k, \kappa_k \right) $ &  57.41 & 60.37 & 61.85 & 58.52 & 61.11 & - & 1 & 500 & 60 \\
$\mathcal{G} \left(  r_{i,j} \mid \alpha_k, \beta_k \right) $ & 41.48 & 40.37 & 42.22 & 39.63 &  36.67 & - & 10 & 1000 & 37.78 \\
$\mathcal{N} \left(  v_{x, i,j}, v_{y,i,j} \mid \boldsymbol{\mu}_k, \boldsymbol{\Sigma}_k \right) $ & 65.93 & 68.15 & 67.04 & 69.63 & 67.41 & - & 100 & 600 & 61.85 \\
$\mathcal{B} \left( \bar{T}_{i,j} \mid \alpha_k, \beta_k \right) \mathcal{VM} \left( \phi_{i,j} \mid \mu_k, \kappa_k \right) $ & 68.89 & 68.89 & 69.63 &  73.33 & 74.44 & 1 & 10 & 650 & $\mathbf{97.41}$ \\
$\mathcal{B} \left(  \bar{T}_{i,j} \mid \alpha_k, \beta_k \right) \mathcal{G} \left( r_{i,j} \mid \alpha_k, \beta_k \right) $ & 51.48 & 48.89 & 49.26 & 52.96 & 49.63 & 1 & 1000 & 650 & 69.26 \\
$\mathcal{VM} \left(  \phi_{i,j} \mid \mu_k, \kappa_k \right) \mathcal{G} \left( r_{i,j} \mid \alpha_k, \beta_k \right) $ & 51.11 & 48.52 & 48.15 & 42.22 & 43.70 & - & 10 & 1000 & 57.78 \\
///////////////////////////////////////////$\mathcal{B} \left(  \bar{T}_{i,j} \mid \alpha_k, \beta_k \right) \mathcal{N} \left( v_{x, i,j}, v_{y,i,j} \mid \boldsymbol{\mu}_k, \boldsymbol{\Sigma}_k \right) $ & 70 & 71.11 & 70.37 & 75.56 & 75.93 & 10 & 1000 & 650 & 94.44 \\   
$\mathcal{B} \left( \bar{T}_{i,j} \mid \alpha_k, \beta_k \right) \mathcal{VM} \left( \phi_{i,j} \mid \mu_k, \kappa_k \right) \mathcal{G} \left(  r_{i,j} \mid \alpha_k, \beta_k \right) $ & 55.19 & 55.19 &  55.56 & 57.41 & 56.3 & 10 & 100 & 1000 & 88.15 \\
$\mathcal{G} \left( \tilde{T}_{i,j} \mid \alpha_k, \beta_k \right) \mathcal{VM} \left( \phi_{i,j} \mid \mu_k, \kappa_k \right) $ & 50.37 &  50.37 &  62.96 & 58.89 & 60 & 10 & 1 & 400 & 67.78 \\
$\mathcal{G} \left( \tilde{T}_{i,j} \mid \alpha_k, \beta_k \right) \mathcal{G} \left( r_{i,j} \mid \alpha_k, \beta_k \right) $ & 62.22 &  62.22 & 50  &  50.37  &  50.74  & 10 & 10 & 400 & 54.81 \\
$\mathcal{G} \left( \tilde{T}_{i,j} \mid \alpha_k, \beta_k \right) \mathcal{VM} \left( \phi_{i,j} \mid \mu_k, \kappa_k \right) \mathcal{G} \left(  r_{i,j} \mid \alpha_k, \beta_k \right) $ & 53.7 & 56.67 & 52.96 & 46.3 & 50.74 & 10 & 1 & 650 & 51.11 \\
$\mathcal{BG} \left( \tilde{T}_{i,j}, r_{i,j} \mid \alpha_k , \beta_k, a_k \right) $ & 50 & 50.37 & 50.37 & 50 & 50.37  & 1 & - & 0 & 50.37 \\
$\mathcal{G} \left( \tilde{T}_{i,j} \mid \alpha_k , \beta_k \right) \mathcal{N} \left( v_{x, i,j}, v_{y,i,j} \mid \boldsymbol{\mu}_k, \boldsymbol{\Sigma}_k \right) $ 
& 61.48 & 61.48 & 62.96 &  55.19 & 57.04 & 1 & 100 & 450 & 68.15 \\
$\mathcal{BG} \left(  \tilde{T}_{i,j}, r_{i,j} \mid \alpha_k, \beta_k, a_k \right) \mathcal{VM} \left( \phi_{i,j} \mid \mu_k, \kappa_k \right) $ & 50 & 50.37 & 50 & 50 & 49.63 & 1 & 1 & 0 & 50 \\
$\mathcal{N} \left(  T_{i,j} \mid \mu_k, \sigma_k \right) \mathcal{VM} \left( \phi_{i,j} \mid \mu_k, \kappa_k \right) $ & $\mathbf{78.15}$ & $\mathbf{76.67}$ & $\mathbf{77.41}$ & 72.96  & 71.85 & 100 & 1000 & 600 & 85.93 \\  
$\mathcal{N} \left(  T_{i,j} \mid \mu_k, \sigma_k \right) \mathcal{G} \left( r_{i,j} \mid \alpha_k, \beta_k \right) $ & 64.07 & 66.67 & 64.44 & 61.85 &  70.37  & 1000 & 100 & 500 & 79.63 \\
$\mathcal{N} \left(  T_{i,j} \mid \mu_k, \sigma_k \right) \mathcal{VM} \left( \phi_{i,j} \mid \mu_k, \kappa_k \right) \mathcal{G} \left( r_{i,j} \mid \alpha_k, \beta_k \right) $ & 73.33 &  67.78 & 68.15 &  72.96 & 68.89 & 100 & 1 & 400 & 72.96 \\
$\mathcal{N} \left(  T_{i,j}, v_{x, i,j}, v_{y,i,j} \mid \boldsymbol{\mu}_k, \boldsymbol{\Sigma}_k \right) $ & 52.22 & 52.96 & 52.22 & 51.85 & 64.44 & 100 & - & 1000 & 74.07 \\
\bottomrule
\end{tabular}
\caption{Detection accuracy achieved for the different probability functions used in the likelihood in a mixture model. The detection accuracy is compared using different Beyesian metrics and a mixture model with a prior on the mixture weights and the cloud layers number.}
\label{tab:mms}

\end{table}
